Model comparison of the dark matter profiles of Fornax, Sculptor, Carina and Sextans

We use orbit based dynamical models to fit the 2nd and 4th moments of the line of sight velocity distributions of the Fornax, Sculptor, Carina and Sextans dwarf spheroidal galaxies. Our goal is to compare dark matter profile models of these four systems using Bayesian evidence. We consider NFW, Einasto and several cored profiles for their dark halos and present the probability distribution functions of the model parameters. When considering each system separately, we find there is no preference for one of these specific parametric density profiles. However, the combined evidence shows that it is unlikely that all galaxies are embedded in the same type of cored profiles of the form \rho_{DM} \propto 1/(1 + r^2)^{\beta/2}, where \beta = 3, 4. For each galaxy, we also obtain an almost model independent, and therefore accurate, measurement of the logarithmic slope of the dark matter density distribution at a radius ~ r_{-3}, i.e. where the logarithmic slope of the stellar density profile is -3. This slope ranges from ~ -1.4 for Fornax to ~ -1.1 for Sextans, both at ~ 1 kpc. All our best fit models essentially have the same mass distribution over a large range in radius (from just below r_{-3} to the last measured data point). This remarkable finding likely implies much stronger constraints on the characteristics that subhalos extracted from cosmological simulations should have in order to host the dSph galaxies around the Milky Way.

==> aas_macros.tex <==
%
%  These Macros are taken from the AAS TeX macro package version 4.0.
%  Include this file in your LaTeX source only if you are not using
%  the AAS TeX macro package and need to resolve the macro definitions
%  in the BibTeX entries returned by the ADS abstract service.
%
%  If you plan not to use this file to resolve the journal macros
%  rather than the whole AAS TeX macro package, you should save the
%  file as ``aas_macros.sty'' and then include it in your paper by
%  using a construct such as:
%	\documentstyle[11pt,aas_macros]{article}
%
%  For more information on the AASTeX macro package, please see the URL
%	http://www.aas.org/publications/aastex.html
%  For more information about ADS abstract server, please see the URL
%	http://adswww.harvard.edu/ads_abstracts.html
%

% Abbreviations for journals.  The object here is to provide authors
% with convenient shorthands for the most "popular" (often-cited)
% journals; the author can use these markup tags without being concerned
% about the exact form of the journal abbreviation, or its formatting.
% It is up to the keeper of the macros to make sure the macros expand
% to the proper text.  If macro package writers agree to all use the
% same TeX command name, authors only have to remember one thing, and
% the style file will take care of editorial preferences.  This also
% applies when a single journal decides to revamp its abbreviating
% scheme, as happened with the ApJ (Abt 1991).
\newcommand\aj{{AJ}}                   % Astronomical Journal
\newcommand\araa{{ARA\&A}}             % Annual Review of Astron and Astrophys
\newcommand\apj{{ApJ}}                 % Astrophysical Journal
\newcommand\apjl{{ApJ}}                % Astrophysical Journal, Letters
\newcommand\apjs{{ApJS}}               % Astrophysical Journal, Supplement
\newcommand\ao{{Appl.~Opt.}}           % Applied Optics
\newcommand\apss{{Ap\&SS}}             % Astrophysics and Space Science
\newcommand\aap{{A\&A}}                % Astronomy and Astrophysics
\newcommand\aapr{{A\&A~Rev.}}          % Astronomy and Astrophysics Reviews
\newcommand\aaps{{A\&AS}}              % Astronomy and Astrophysics, Supplement
\newcommand\azh{{AZh}}                 % Astronomicheskii Zhurnal
\newcommand\baas{{BAAS}}               % Bulletin of the AAS
\newcommand\jrasc{{JRASC}}             % Journal of the RAS of Canada
\newcommand\memras{{MmRAS}}            % Memoirs of the RAS
\newcommand\mnras{{MNRAS}}             % Monthly Notices of the RAS
\newcommand\pra{{Phys.~Rev.~A}}        % Physical Review A: General Physics
\newcommand\prb{{Phys.~Rev.~B}}        % Physical Review B: Solid State
\newcommand\prc{{Phys.~Rev.~C}}        % Physical Review C
\newcommand\prd{{Phys.~Rev.~D}}        % Physical Review D
\newcommand\pre{{Phys.~Rev.~E}}        % Physical Review E
\newcommand\prl{{Phys.~Rev.~Lett.}}    % Physical Review Letters
\newcommand\pasp{{PASP}}               % Publications of the ASP
\newcommand\pasj{{PASJ}}               % Publications of the ASJ
\newcommand\qjras{{QJRAS}}             % Quarterly Journal of the RAS
\newcommand\skytel{{S\&T}}             % Sky and Telescope
\newcommand\solphys{{Sol.~Phys.}}      % Solar Physics
\newcommand\sovast{{Soviet~Ast.}}      % Soviet Astronomy
\newcommand\ssr{{Space~Sci.~Rev.}}     % Space Science Reviews
\newcommand\zap{{ZAp}}                 % Zeitschrift fuer Astrophysik
\newcommand\nat{{Nature}}              % Nature
\newcommand\iaucirc{{IAU~Circ.}}       % IAU Cirulars
\newcommand\aplett{{Astrophys.~Lett.}} % Astrophysics Letters
\newcommand\apspr{{Astrophys.~Space~Phys.~Res.}}
                % Astrophysics Space Physics Research
\newcommand\bain{{Bull.~Astron.~Inst.~Netherlands}} 
                % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{{Fund.~Cosmic~Phys.}}  % Fundamental Cosmic Physics
\newcommand\gca{{Geochim.~Cosmochim.~Acta}}   % Geochimica Cosmochimica Acta
\newcommand\grl{{Geophys.~Res.~Lett.}} % Geophysics Research Letters
\newcommand\jcp{{J.~Chem.~Phys.}}      % Journal of Chemical Physics
\newcommand\jgr{{J.~Geophys.~Res.}}    % Journal of Geophysics Research
\newcommand\jqsrt{{J.~Quant.~Spec.~Radiat.~Transf.}}
                % Journal of Quantitiative Spectroscopy and Radiative Transfer
\newcommand\memsai{{Mem.~Soc.~Astron.~Italiana}}
                % Mem. Societa Astronomica Italiana
\newcommand\nphysa{{Nucl.~Phys.~A}}   % Nuclear Physics A
\newcommand\physrep{{Phys.~Rep.}}   % Physics Reports
\newcommand\physscr{{Phys.~Scr}}   % Physica Scripta
\newcommand\planss{{Planet.~Space~Sci.}}   % Planetary Space Science
\newcommand\procspie{{Proc.~SPIE}}   % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
